Blackboard Rules for Coordinating Context-aware Applications in Mobile Ad Hoc Networks

Thanks to improvements in wireless communication technologies and increasing computing power in hand-held devices, mobile ad hoc networks are becoming an ever-more present reality. Coordination languages are expected to become important means in supporting this type of interaction. To this extent we argue the interest of the Bach coordination language as a middleware that can handle and react to context changes as well as cope with unpredictable physical interruptions that occur in opportunistic network connections. More concretely, our proposal is based on blackboard rules that model declaratively the actions to be taken once the blackboard content reaches a predefined state, but also that manage the engagement and disengagement of hosts and transient sharing of blackboards. The idea of reactiveness has already been introduced in previous work, but as will be appreciated by the reader, this article presents a new perspective, more focused on a declarative setting.

==> eptcsdata.tex <==
\providecommand{\firstpage}{63}
\providecommand{\publicationstatus}{Natallia Kokash and Ant\'onio Ravara (Eds.): 11th International Workshop on\\ Foundations of Coordination Languages and Self Adaptation (FOCLASA'12)\\
EPTCS 91, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.91.5}{10.4204/EPTCS.91.5}}
\pdfoutput=1

